Minimax Least-Square Policy Iteration for Cost-Aware Defense of Traffic Routing against Unknown Threats

Dynamic routing is one of the representative control scheme in transportation, production lines, and data transmission. In the modern context of connectivity and autonomy, routing decisions are potentially vulnerable to malicious attacks. In this paper, we consider the dynamic routing problem over parallel traffic links in the face of such threats. An attacker is capable of increasing or destabilizing traffic queues by strategic manipulating the nominally optimal routing decisions. A defender is capable of securing the correct routing decision. Attacking and defensive actions induce technological costs. The defender has no prior information about the attacker's strategy. We develop an least-square policy iteration algorithm for the defender to compute a cost-aware and threat-adaptive defensive strategy. The policy evaluation step computes a weight vector that minimizes the sampled temporal-difference error. We derive a concrete theoretical upper bound on the evaluation error based on the theory of value function approximation. The policy improvement step solves a minimax problem and thus iteratively computes the Markov perfect equilibrium of the security game. We also discuss the training error of the entire policy iteration process.

==> Texts/Game.tex <==
\section{Security game}

An attacker is able to launch jamming attacks at random times. Specifically, attacks occur with a Poisson rate of $\lambda$. The attacker is able to select the value of $\lambda$ out of the interval $[0,\bar\lambda]$, where $\bar\lambda>0$ is the budget for the attacker. The utility $u_1$ for the attacker is given by
\begin{align*}
    u_1(\lambda,r)=\bar X(\lambda,r)-f(\lambda),
\end{align*}
where $f(\lambda)$ is the attack cost function.
We assume the following for the cost function.
\begin{asm}
We assume that $f:[0,\bar\lambda]\to\mathbb R_{\ge0}$ is non-decreasing in $\lambda$ and such that $\lim_{\lambda\to\bar\lambda}f(\lambda)=\infty$.
\end{asm}
The assumption of non-decreasing is intuitive: more attacks induce more costs. The assumption of the infinite limit 

The system operator (SO) selects the admitted load $r$ of the system. The utility $u_1$ for the SO is given by
\begin{align*}
    u_2(\lambda,r)=-\bar X(\alpha,b)+c_2r.
\end{align*}

==> Texts/Model.tex <==
\section{Introduction}
\label{sec_model}

Platooning of connected and autonomous vehicles (CAVs) has the potential for remarkable efficiency and environmental benefits. The idea of automatically regulating a string of vehicles is well-known, and extensive experimental studies in real-world traffic conditions have been conducted. However, in spite of recent progress in vehicle-level control design and system-level simulations, the interaction   between CAV platoons and the background traffic on the highway has not been well understood, and, consequently, the management of platoons on mixed-traffic highways has not been well studied. This is one of the most important question that needs addressing before extensive deployment of the platooning technology, since CAV platoons are essentially moving bottlenecks for the background traffic and limited highway capacity should be shared between these two classes of traffic in an appropriate manner. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper, we develop a cooperative control strategy that regulates the travel time of platoons on a mixed-traffic highway section. We consider a typical setting as shown in Fig. 1. The highway segment is constrained by a downstream bottleneck. Congestion initiated at the bottleneck may impede the movement of exiting vehicles(i.e. spillback); this is the major source of efficiency loss.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
One way of resolving such spillback is to regulate the travel time of platoons so that they arrive at the bottleneck with relatively evenly distributed moments; Although this idea is simple and intuitive, implementation faces several challenges. First, travel-time regulation involves deceleration of some platoons, which induces delay on the platoon itself as well as the surrounding background traffic; therefore, it is essential to avoid “over-deceleration”. Second, performance of any travel-time regulation strategy depends on the interaction between platoons and the background traffic; however, microscopic models, although realistic, are overly complex for calibration, control design, and real-time implementation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To address the above challenges, we study the modeling, analysis and control methodology of the road segment system. In order to reflect the interaction mechanism between CAVs and non-CAVs and the remaining passage time of each vehicle in the model, we construct a hybrid queuing model represented by temporal cells to solve the modeling problem. Based on the concept of system state equation in modern control theory, the state equations of the road segment system are established, and the system performance is analyzed. In order to maximize road traffic efficiency, the cooperative control strategy is designed, and the control methodology of vehicle-vehicle cooperation and vehicle-road cooperation at the macro level of the system is theoretically provided.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Our work also involves a well-known micro-simulation tool called Simulation of Urban MObility (SUMO). SUMO is a standard traffic simulation package and has been used for study on platooning. We essentially view the hybrid queuing model as a reduced-order model for the micro-simulation model in that the queuing model captures the aggregate queuing delay due to platooning-induced flow fluctuation. We find that although the queuing model drops certain details from the micro-simulation, it adequately predicts the aggregate behavior of traffic under the influence of platoons.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The rest of this paper is organized as follows. In Section ??, we introduce the models ??. In Section ??, we analyse the performance and design cooperative control strategy??. In Section ??, simulation and verification??. In Section ??, we summarize the main results and mention several directions of future work that are theoretically interesting and/or practically relevant.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Modeling and formulation}
In this section, we set relevant parameters and introduce our temporal-cell model for the platoon coordination problem ??. We consider a queuing model with non-zero traverse time and with capacity drop (breakdown). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Environment}
A typical road section setting is shown in Figure 1. There is a bottleneck at the downstream.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htp]
    \centering
    \includegraphics[width=7cm]{Images/f1.png}
    \caption{road section with downstream bottleneck}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
1. Background traffic demand \(a(t)\in R\geq 0\): the number of non-CAVs entering the highway section during the \(t\)th time step. If environmental information is known, such as road type, weather and time of day, \(a(t)\)will be a constant \(\bar {a}\).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
2. CAV demand  \(B(t)\in Z\geq 0\): the size of the CAV platoon entering the highway section during the \(t\)th time step. The platoon size follows geometric distribution, \(Pr\left\{B(t)=b \right\}=p_B(b)=\beta (1-\beta )^b\),\(b=0,1,2,3...,\beta\in\left( 0,1\right)\). We assume no more than one platoon during each time step, since if multiple platoons arrive during a sufficiently small time interval, then these platoons can probably merge into one. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A malicious attacker is able to launch jamming attack at the V2I communication network for the intersection. The attacks occur at random times with Poisson rate $\lambda\ge0$. During an attack, the attacker induces a communication delay of $\theta>0$. The attacker terminates an attack at a Poisson rate of $\mu>0$.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Capacity model}

% Liu et al. used a trajectory-based model to show that the intersection's capacity can be approximated by the following formula \cite{liu2021latency}:
% \begin{align*}
%     f(y)=\frac{\bar v}{2\epsilon(y+\delta)+\bar v},
% \end{align*}
% where $\bar v$ is the crossing speed, $\epsilon$ is the kinematic uncertainty, $\delta$ is the time step size.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Queuing delay model}

% In the presence of jamming attacks, the behavior of the traffic queue can be described by the piecewise-deterministic queuing (PDQ) model. That is, let $X(t)$ be the total queue size at time $t$ and let $Y(t)$ be the latency at time $t$. Then, the PDQ is a hybrid-state process with state $(X(t),Y(t))$ and state space $\mathbb R_{\ge0}\times\{0,\theta\}$.

% The discrete state $Y(t)$ evolves according to a two-state Markov process with transition rates $\lambda$ and $\mu$; see Fig.~\ref{}. The continuous state $X(t)$ evolves according to the following differential equation:
% \begin{align*}
%     \frac d{dt}X(t)=\begin{cases}
%     r-f(Y(t)) & X(t)>0,\\
%     \Big(r-f(Y(t))\Big)_+ & X(t)=0.
%     \end{cases}
% \end{align*}

% One can obtain an analytical expression for the long-time average queuing delay \cite{jin2018modeling}:
% \begin{align*}
%     \bar X(\lambda,r)=\begin{cases}
%     0 & \mbox{if }r\le f',\\
%     \frac{\lambda}{\mu}\frac{(f'-f)r+f'(f-f')}{\lambda(r-f')+\mu(r-f)} & \mbox{otherwise.}
%     \end{cases}
% \end{align*}

==> Texts/beiyong.tex <==
% The observation of the attacking cost $c_a$ is specified by $o_c(s,u) \in \mathbb{R^+}$. The corresponding estimated value is $c_a$ which is sampled from a probability distribution based on past actions and observations, known as the \textit{belief}. The belief $b_{t+1}(\hat c_a|o_c)$ at time t+1 can be computed from the previous belief $b_t(\hat c_a|o_c)$, the last action $u$ and observation $o$, according to the beyesian rule. The prior distribution of $\hat c_a$ is considered as a uniform distribution with constant parameters zero and $C$. Define the marginal distribution of observation $o_c$ as $m(o_c)=\int_{C}b_t(o_c|\hat c_a)g(\hat c_a) d\hat c_a $
% \begin{align*}
%     b_{t+1}(\hat c_a|o_c)=\frac{b_t(o_c|\hat c_a)*g(\hat c_a)}{m(o_c)}
% \end{align*}
% Based on Maximum A Posteriori in Bayesian statistics, the best estimated attacker cost $\hat c_a$ at time $t$ can be calculated as follows:
% \begin{align*}
%     \hat c_a &= \arg\max_{\hat c_a} b_t(o_c|\hat c_a)*g(\hat c_a)\\
%     &=\arg\max_{\hat c_a}\prod_{i=1}^{n}b_t(o_c^i|\hat c_a)*g(\hat c_a)\\
%     &=\arg\max_{\hat c_a}\sum_{i=1}^{n}\log b_t(o_c ^i|\hat c_a) + \log g(\hat c_a)
% \end{align*}
% where $n$ denotes the number of collected data.

We are motivated to verify if the defender can learn a MPE strategy given the attacker's static strategy. In the context of imperfect information, which is normal scenarios for defender, we assume the attacker is well-known and attempt to implement best attack policy $a^*$. Then the interaction can be reformulated as a Markov Decision Process for defender. %plan to use Q-learning, if can learn best response in this worst case, it's probably to give defender advantage to deal with other better situations.

For every state-action pair $(x,u)$, the estimated immediate reward $\hat R(x,u)$ obeys discrete probability as follows, if attacker uses static strategy.
\begin{align*}
    \begin{cases}
P(\hat R(x,u)=&\Vert x' \Vert_{1}+c_b 1\{u=P\}-\hat c_a)=a^*(x) \quad \mbox{if }a=A,\\
P(\hat R(x,u)=&\Vert x' \Vert_{1}+c_b 1\{u=P\})=(1-a^*(x)) \quad \mbox{if }a=NA
    \end{cases}
\end{align*}

We use the mean of the reward sequence ${R_k}$ in iteration, which can be computed incrementally:
\begin{align*}
    \overline{R}&=\frac{1}{k} \sum_{i=1}^{k} R_i\\
    &=\frac{1}{k}(R_k+\sum_{i=1}^{k-1} R_i)\\
    &=\frac{1}{k}[R_k+(k-1)\overline{R}_{k-1}]\\
    &=\overline{R}_{k-1}+\frac{1}{k}(R_k-\overline{R}_{k-1})
\end{align*}
According to Lemma 1, $\overline{R}$ will converge to mean $\overline{X}=\mathbb{E}[R]=a^* R^A+(1-a^*)R^{NA}$.The $R^A$ refers to rewards when attack is taken while $R^{NA}$ refers to the opposite.

The iteration of $Q_t$ can be rewritten as follows.
\begin{equation} %加*表示不对公式编号
    \begin{split}
        Q_{t+1}(x,u)
         &=\\ [1-\alpha(t)]&Q_{t}(x,u)+\alpha(t)[\hat R(x',u) + \gamma \min_{v \in U(x')} Q_{t}(x',v)]
        \\=[1-\alpha(t)]&Q_{t}(x,u)+\alpha(t)[FQ_{t}(x,u)+w(x,u)]
   \end{split}
\end{equation} 
with the operator $F$ defined as:
\begin{align*}
    FQ_{t}(x,u)=\mathbb{E}[\hat R(x',u)+\gamma \min_{v \in U(x')} Q_{t}(x',v)|\mathcal{F}_t]
\end{align*}
The operator is based on the history of the algorithm $\mathcal{F}_t$ which consists of attacker's action $(a_k)_{k \leq t}$ up to time $t$. The noise term is defined as:
\begin{align*}
    w(x,u):&=\hat R(x',u) + \gamma \min_{v \in U(x')} Q_{t}(x',v) - FQ_t(x,u)\\
    &=\hat R(x',u)-\mathbb{E}[\hat R(x',u)] + \gamma \min_{v \in U(x')} Q_{t}(x',v) \\&- \gamma \mathbb{E}[\min_{v \in U(x')} Q_{t}(x',v)|\mathcal{F}_t]
\end{align*}

\begin{align*}
   &\Vert FQ-FQ' \Vert_{\infty}\\
   =&\max_{x,u}\vert \mathbb{E}[\hat R(x',u)+\gamma \min_{v} Q_{t}(x',v)|\mathcal{F}_t]\\&-\mathbb{E}[\hat R(x',u)+\gamma \min_{v} Q'_{t}(x',v)|\mathcal{F}_t]
   \vert \\
   =&\max_{x,u}\vert \mathbb{E}[\hat R(x',u)+\gamma \min_{v} Q_{t}(x',v)|xu]\\&-\mathbb{E}[\hat R(x',u)+\gamma \min_{v} Q'_{t}(x',v)|xu]
   \vert\\
   \leq &\max_{x,u} \min_{x'} \gamma\vert \min_{v} Q_{t}(x',v)-\min_{v} Q'_{t}(x',v)\vert\\
   \leq &\gamma \max_{x,u} \vert Q_{t}(x',v)-Q'_{t}(x',v) \vert\\
   =& \gamma \Vert Q-Q' \Vert_{\infty}
\end{align*}

By the Bellman Optimality equation:
\begin{align*}
    &V^*(x)= \min_{u} Q^*(x,u)\\
    &Q^*(x,u)= \overline{R}(x,u) + \gamma \sum_{x'}P(x'|x,u) V^*(x')
\end{align*}
Then
\begin{align*}
    FQ^*(x,u)&=\mathbb{E}[\hat{R}(x,u) + \gamma \min_{v} Q^*(x',v)]\\
    &=\sum_{x'}P(x'|x,u)[\hat{R}(x,u) + \gamma \min_{v} Q^*(x',v)]\\
    &=\overline{R}(x,u) + \gamma \sum_{x'}P(x'|x,u) \min_{v} Q^*(x',v)\\
    &=\overline{R}(x,u) + \gamma \sum_{x'}P(x'|x,u) V^*(x')\\
    &=Q^*(x,u)
\end{align*}
So $F$ has a fixed point $Q^*$ with the same contraction factor $\gamma$.
\begin{align*}
    \Vert FQ-Q^* \Vert_{\infty}=\Vert FQ-FQ^* \Vert_{\infty} \leq \gamma\Vert Q-Q^* \Vert_{\infty}
\end{align*}

The mean value of the noise is zero.
\begin{align*}
    \mathbb{E}[w(x,u)|\mathcal{F}_t]&=\\
    \mathbb{E}[\hat R(x',u) &+ \gamma \min_{v} Q_{t}(x',v) - FQ_t(x,u)|\mathcal{F}_t]=0
\end{align*}
The variance of the noise is bounded under Assumption 2.
\begin{align*}
    \mathbb{E}[w(x,u)^2|\mathcal{F}_t]&=
    \mathbb{E}[(\hat R(x',u) + \gamma \min_{v} Q_{t}(x',v))^2|\mathcal{F}_t] \\&- \mathbb{E}[\hat R(x',u) + \gamma \min_{v} Q_{t}(x',v)|\mathcal{F}_t]^2\\&
    \leq \frac{1}{4}[\max_{x'R}(\hat R(x',u)+\gamma \min_{v} Q_{t}(x',v))\\&-\min_{x'R}(\hat R(x',u)+\gamma \min_{v} Q_{t}(x',v))]^2\\&
    \leq \frac{1}{4}(\frac{R_{max}-R_{min}}{1-\gamma}+\gamma \Vert Q_t \Vert_{\infty})^2\\&
    =\frac{1}{4}(\Delta^2+2\gamma\Delta\Vert Q_t \Vert_{\infty}+\gamma^2\Vert Q_t \Vert_{\infty}^2) \\&
    \leq A+B\Vert Q_t \Vert_{\infty}^2
\end{align*}
where constant $\Delta=(R_{max}-R_{min})/(1-\gamma)$. $\Vert \cdot \Vert_{\infty}$ means sup-norm and $\Vert Q_t \Vert_{\infty}$ is bounded by some constant $C$ according to Assumption 2. Then $A=\frac{1}{4}\Delta^2+\frac{C\gamma}{2}\Delta$ and $B=\frac{\gamma^2}{4}$.

Under Assumption 1 and 2, for each $(x,u) \in X \times U$, the sequence $(Q_t)_{t\in \mathbb{N}}$ generated by the iteration converges to $Q^*$.

We have all the conditions to invoke a convergence result from Bertsekas and Tsitsiklis [1995]. We adopt and state
Proposition 4.5 from Bertsekas and Tsitsiklis [1995] without reproducing the complete proof.

To verify if the strategy profile is a MPE, we should first verify the Markov property of the strategy. Then check whether it is a subgame-perfect euilibrium with the single-deviation principle.

At each time-step $t$, the defender in a state $x:=x(t)$ takes an action $u:=u(t)$ and receives an estimated reward $\hat R(x,u)$ based on $\hat c_a$ and the next state $x:=x(t+1)$. Then the defender performs an action-value update to the $(x,u)$-estimate with the following Q-learning update rule:
\begin{align*}
    Q_{t+1}(x,u,a)&=Q_{t}(x,u,a)\\+\alpha(t)[\hat R(x',u,a) &+ \gamma \min_{v \in U(x')} Q_{t}(x',v,a')-Q_{t}(x,u,a')]
\end{align*}
where $(\alpha(t))_{t\in \mathbb{N}}$ is a learning rate sequence.

